Localizing Memorization in SSL Vision Encoders

Recent work on studying memorization in self-supervised learning (SSL) suggests that even though SSL encoders are trained on millions of images, they still memorize individual data points. While effort has been put into characterizing the memorized data and linking encoder memorization to downstream utility, little is known about where the memorization happens inside SSL encoders. To close this gap, we propose two metrics for localizing memorization in SSL encoders on a per-layer (layermem) and per-unit basis (unitmem). Our localization methods are independent of the downstream task, do not require any label information, and can be performed in a forward pass. By localizing memorization in various encoder architectures (convolutional and transformer-based) trained on diverse datasets with contrastive and non-contrastive SSL frameworks, we find that (1) while SSL memorization increases with layer depth, highly memorizing units are distributed across the entire encoder, (2) a significant fraction of units in SSL encoders experiences surprisingly high memorization of individual data points, which is in contrast to models trained under supervision, (3) atypical (or outlier) data points cause much higher layer and unit memorization than standard data points, and (4) in vision transformers, most memorization happens in the fully-connected layers. Finally, we show that localizing memorization in SSL has the potential to improve fine-tuning and to inform pruning strategies.

==> content/06_discussion.tex <==
\section{Discussion and Future Work}

\subsection{Insights into SSL Memorization}
\citep{wang2021chaos}
-- 4) Can we relate the augmentation strength to the instance selectivity theoretically?
contrastive SSL optimizes for uniformity, i.e., a uniform distribution of samples over the representation space~\citep{wang2020understanding}. -- potentially, this uniformity in feature space can be achived through having units memorize particular instances.

\subsection{What can our metric do?}
Future work may benefit by using our \unitmem metric for finding which units within a network can be removed while preserving or maintaining high performance (\textbf{pruning}). Given any trained model, we iteratively remove filters corresponding to selected units. We set three different criteria for the removal based on most memorized, least memorized, and randomly chosen units. We observe that discarding the most memorized units leads to the highest drop in accuracy on a downstream task.  

Our metric can also be used for white-box privacy attacks where the attacker exploits the memorization of individual data points in individual units.


